Empowering Sentence Encoders with Prompting and Label Retrieval for Zero-shot Text Classification

With contrastive pre-training, sentence encoders are generally optimized to locate semantically similar samples closer to each other in their embedding spaces. In this work, we focus on the potential of their embedding spaces to be readily adapted to zero-shot text classification, as semantically distinct samples are already well-separated. Our framework, RaLP (Retrieval augmented Label Prompts for sentence encoder), encodes prompted label candidates with a sentence encoder, then assigns the label whose prompt embedding has the highest similarity with the input text embedding. In order to compensate for the potentially poorly descriptive labels in their original format, RaLP retrieves sentences that are semantically similar to the original label prompt from external corpora and use them as additional pseudo-label prompts. RaLP achieves competitive or stronger performance than much larger baselines on various closed-set classification and multiple-choice QA datasets under zero-shot settings. We show that the retrieval component plays a pivotal role in RaLP's success, and its results are robustly attained regardless of verbalizer variations.

==> Sections/tables/algorithm.tex <==
% \begin{algorithm}[tb] 
% % \small
%  \caption{Pseudo Code for Retrieval Augmented Label Prompt}
%  \label{alg:tess_r}
% \begin{algorithmic}[1]
  
%   \STATE \textbf{Input}: class index  $y=\{y_1,...,y_{m}\}$; external corpus $ \textbf{C}$;
%               \\~~~~~~~~~~ verbalizer map $v$ expansion $\textbf{D}$;
%   \STATE \textbf{Output}: lists of augmented samples $\hat{y}= \{\hat{y}_{1}...,\hat{y}_{m}\}$.
%   % \\~~~~~~~~~~~~~ $\hat{y}= \{\hat{y}_{1}...,\hat{y}_{m}\}$.

%   \STATE Initialize hyperparamenters $k, e$.
%   \STATE Initialize Empty list $\hat{y}$.
%   \FOR{$i$ in [1, 2, ..., m]}
%   \STATE $v_E= Glove(y_{i},\textbf{D},e) $ $\gets $ \COMMENT{find verbalizers.}

%   \FOR{$v_e$ in [$v_1$, $v_2$, ..., $v_E$]}
%   \STATE  \hat{y}^e_i= \textbf{topk}($v_e(y_i)$,$\textbf{C}$,$k$) $\gets$ \COMMENT{retrieving $k$ examples from external corpus $\textbf{C}$ using verbalizer map $v_e$}
%   \STATE $\hat{y}$.append($\hat{y}$^e_i)
%   \ENDFOR
%   \ENDFOR
  
%   \RETURN $\hat{y}$

% \end{algorithmic}
% \end{algorithm}
% % 

==> Sections/tables/fewshot_comparison.tex <==
\begin{table*}[t]
\centering
% \small
\resizebox{1.0\textwidth}{!}{
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{|l|cc|cc|cc|cc|}
\toprule
        & \multicolumn{2}{c|}{\textbf{4-shot}}                                                 & \multicolumn{2}{c|}{\textbf{8-shot}}                                                  & \multicolumn{2}{c|}{\textbf{16-shot}}                                                & \multicolumn{2}{c|}{\textbf{0-shot}}                               \\
\hline
\textbf{Dataset} & \textbf{Linear Probing}                           & \textbf{ProtoType}                                & \textbf{Linear Probing}                            & \textbf{ProtoType}                                & \textbf{Linear Probing}                           & \textbf{ProtoType}                                & \textbf{TeSS}     & \textbf{TeSS-R}   
\\
\hline
\textbf{SST-2}   & 84.7$_\text{3.5}$ / 74.3 & 84.8$_\text{3.5}$ / 73.9 & 88.3$_\text{1.7}$ / 83.8 & 88.1$_\text{1.7}$ / 83.6 & 89.7$_\text{1.0}$ / 87.3 & 89.8$_\text{0.9}$ / 87.5 & 87.7 & 87.6 \\
\hline
\textbf{MR}      & 77.9$_\text{4.5}$ / 64.3 & 78.0$_\text{4.6}$ / 62.5 & 82.0$_\text{2.6}$ / 73.7  & 82.0$_\text{2.6}$ / 71.8 & 84.1$_\text{1.1}$ / 81.5 & 84.3$_\text{0.9}$ / 82.6 & 81.7 & 81.4 \\
\hline
\textbf{CR}      & 50.0$_\text{0.0}$ / 50.0 & 71.9$_\text{9.6}$ / 51.4 & 50.0$_\text{0.0}$ / 50.0  & 77.9$_\text{7.3}$ / 57.0 & 50.0$_\text{0.0}$ / 50.0 & 87.1$_\text{3.0}$ / 79.8 & 87.3 & 87.2 \\
\hline
\textbf{RT}      & 78.0$_\text{4.6}$ / 61.0 & 78.2$_\text{4.6}$ / 60.7 & 82.1$_\text{2.2}$ / 77.0  & 81.9$_\text{2.5}$ / 73.7 & 84.3$_\text{1.2}$ / 81.8 & 84.3$_\text{1.3}$ / 79.6 & 81.9 & 82.1 \\
\hline
\textbf{Yahoo}   & 45.5$_\text{3.5}$ / 37.1 & 44.1$_\text{3.4}$ / 36.7 & 41.1$_\text{2.2}$ / 36.2  & 54.5$_\text{2.3}$ / 50.2 & 57.8$_\text{1.7}$ / 54.2 & 60.9$_\text{1.8}$ / 57.4 & 55.3 & 57.7 \\
\hline
\textbf{AGNews}  & 70.4$_\text{4.2}$ / 59.0 & 69.7$_\text{4.4}$ / 58.2 & 77.6$_\text{2.7}$ / 68.9  & 76.8$_\text{3.1}$ / 66.1 & 81.1$_\text{1.6}$ / 77.7 & 81.4$_\text{1.9}$ / 76.8 & 70.4 & 76.9 \\
\bottomrule
\end{tabular}

}
\caption{Fewshot versus Zeroshot Comparison.}

\end{table*}



==> Sections/tables/scaling_law_table.tex <==
% \begin{table}[t]
% \centering
% % \small
% \renewcommand{\arraystretch}{1.1}
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{lrcccccccc}
% \toprule
% \textbf{Method} & \textbf{\# Params} & \textbf{SST-2} & \textbf{MR} & \textbf{CR} &  \textbf{RT} & \textbf{Yahoo} & \textbf{AGNews} & \textbf{Avg}\\
% \hline
% \ours$_\text{ST5-B}$   & 110M & 84.0 & 78.2 & 86.4 & 78.3 &	50.9 & 73.9 & 75.3	 \\
% $\textit{+R}$          & 110M & 84.2 & 78.0 & 86.7 & 78.2 & 56.3 & 78.5 & 77.0 \\
% \ours$_\text{ST5-L}$   & 335M & 87.7& 81.7        & 87.3        & 81.9        & 55.3& 70.4    &77.4 \\
% $\textit{+R}$          & 335M & 87.6 & 81.4        & 87.2   & 82.1        & 57.7& 76.9   & 78.9 \\
% \ours$_\text{ST5-XL}$   & 1.25B & 89.0 & 82.9 & 86.2  & 83.3  & 53.5 & 71.4  & 77.7  \\
% $\textit{+R}$           & 1.25B & 88.6 & 82.8 & 86.1  & 83.3  & 56.2 & 75.1  & 78.7 \\
% \ours$_\text{ST5-XXL}$  & 4.8B & 89.7 & 84.0 & 87.7   & 84.5  & 53.6 & 71.0  & 78.4 \\
% $\textit{+R}$           & 4.8B & 90.5 & 84.7 & 87.7   & 85.1  & 54.9 & 75.4  & 79.7    \\
% \bottomrule
% \end{tabular}
% }
% \caption{Scaling Law
% }
% \label{tab:scaling_law}
% \end{table}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.7\linewidth]{Sections/figures/ver1.jpg}
% \caption{Macro averaged accuracy according to model scale. \bokyung{add legend (color)}
% }
% \label{fig:scale}
% \end{figure}





==> Sections/tables/tess_setup.tex <==
\begin{table}[h]
    \begin{adjustbox}{width=0.47\textwidth}
        \begin{tabular}{lcc}
            \toprule
            Variation         & Training Corpus   & \# of Params \\
            \hline
            \ours$_\text{SimCSE}$   & NLI       & 355M\\
            \ours$_\text{ST5}$ & CommunityQA + NLI & 335M \\       
            \ours$_\text{ST5-XL}$ & CommunityQA + NLI & 1.25B \\       
            \ours$_\text{ST5-XXL}$ & CommunityQA + NLI & 4.8B \\       
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\caption{The details of \ours~variation.}
\label{tab:tess_setup}
\end{table}
\vspace{-1.0ex}
